DialogStudio: Towards Richest and Most Diverse Unified Dataset Collection for Conversational AI

Despite advancements in conversational AI, language models encounter challenges to handle diverse conversational tasks, and existing dialogue dataset collections often lack diversity and comprehensiveness. To tackle these issues, we introduce DialogStudio: the largest and most diverse collection of dialogue datasets, unified under a consistent format while preserving their original information. Our collection encompasses data from open-domain dialogues, task-oriented dialogues, natural language understanding, conversational recommendation, dialogue summarization, and knowledge-grounded dialogues, making it an incredibly rich and diverse resource for dialogue research and model training. To further enhance the utility of DialogStudio, we identify the licenses for each dataset, design external knowledge and domain-aware prompts for selected dialogues to facilitate instruction-aware fine-tuning. Furthermore, we develop conversational AI models using the dataset collection, and our experiments in both zero-shot and few-shot learning scenarios demonstrate the superiority of DialogStudio. To improve transparency and support dataset and task-based research, as well as language model pre-training, all datasets, licenses, codes, and models associated with DialogStudio are made publicly accessible\footnote{\url{https://github.com/salesforce/DialogStudio}}.

==> Tex/dataset.tex <==
\section{Datasets} \label{sec:data}
We collect and process in total 65 datasets, covering task-oriented dialogs, conversational recommendation, dialog summarization, and dialog rewriting. There are in total more than one million dialogs, involving different domains, dialog types, and dialog tasks.
\subsection{Task-Oriented Dialogue Datasets}
There are total of 28 task-related dialog datasets in our collection, as shown in Tab.~\ref{tab:data}. 
% split
We conduct the train/val/test split based on their original split strategy. If there is no pre-defined split strategy, we consider the whole dataset as the training set.

% prompt
We manually pre-define five different prompt templates, such as "This is a bot helping users to $\_\_\_$ . Given the dialog context and external database, please generate a relevant system response for the user." For each domain, we also write a corresponding description, e.g. "restaurants": "find and book a restaurant". Therefore, for each dialog, we sample a prompt template and fill in the combination of domain descriptions, corresponding to its involved domains.



% \subsubsection{format}
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Tex/Figs/data.png}
\caption{Datasets from the Task-Oriented Dialog Subcollection} 
\label{fig:data}
\end{figure}

% \begin{itemize}
%     \item table to list all dataset
%     \item example
% \end{itemize}

% % \begin{table}[]
% \small
% \begin{tabular}{p{2cm}|p{5cm}|p{1cm}|p{1cm}|p{1cm}|l}
% \toprule
% \multicolumn{1}{l|}{}                         & Datasets                                       & Train                        & Valid                     & Test                      & Database                  \\ \cline{2-6} 
% \multirow{9}{*}{\textbf{NLU}}                  & NLU++                                          & 3080                         &                           &                           &                           \\ \cline{2-6} 
%                                                & BANKING77                                      & 8622                         & 1540                      & 3080                      &                           \\ \cline{2-6} 
%                                                & RESTAURANT8K (Slot Filling)                    & 7244                         & 1000                      & 3731                      &                           \\ \cline{2-6} 
%                                                & CLINC150                                       & 15000                        & 3000                      & 4500                      &                           \\ \cline{2-6} 
%                                                & HWU64                                          & 8954                         & 1076                      & 1076                      &                           \\ \cline{2-6} 
%                                                & SNIPS                                          & 13084                        & 700                       & 700                       &                           \\ \cline{2-6} 
%                                                & DSTC8-SGD (Slot Filling)                       & 5023                         & 602                       & 1813                      &                           \\ \cline{2-6} 
%                                                & TOP (SP)                                       & 31279                        & 4462                      & 9042                      &                           \\ \cline{2-6} 
%                                                & ATIS                                           &                              &                           &                           &                           \\ \cline{1-6} 
% \multirow{28}{*}{\textbf{TOD}}                 & MultiWOZ 2.2                                   & 8438                         & 1000                      & 1000                      & Y                         \\ \cline{2-6} 
%                                                & KVRET                                          & 2425                         & 302                       & 304                       & Y                         \\ \cline{2-6} 
%                                                & WOZ 2.0                                        & 600                          & 200                       & 400                       &                           \\ \cline{2-6} 
%                                                & DSTC2-CLEAN                                    & 1612                         & 506                       & 1117                      & Ontology                  \\ \cline{2-6} 
%                                                & FRAMES                                         & 1369                         & N/A                       & 40                        & KB                        \\ \cline{2-6} 
%                                                & SGD                                            & 16142                        & 2482                      & 4201                      & Ontology                  \\ \cline{2-6} 
%                                                & MulDoGo                                        & 40576                        &                           &                           &                           \\ \cline{2-6} 
%                                                & TaskMaster1                                    &                              &                           &                           & \multirow{3}{*}{Ontology} \\ \cline{2-5}
%                                                & TaskMaster2                                    &                              &                           &                           &                           \\ \cline{2-5}
%                                                & TaskMaster3                                    &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & BiTOD                                          & 2952                         & 295                       & 442                       & Y                         \\ \cline{2-6} 
%                                                & SimJoint-Movie                                 & 1116                         & 349/120                   & 775/264                   & \multirow{3}{*}{N/A}      \\ \cline{2-5}
%                                                & SimJoint-Restaurant                            &                              &                           &                           &                           \\ \cline{2-5}
%                                                & SimJoint-GEN                                   & \textbf{100K}                & 10K                       & 10K                       &                           \\ \cline{2-6} 
%                                                & AirDialogue                                    & 321,460                      & 40,363                    & 40,215                    & KB                        \\ \cline{2-6} 
%                                                & MIT-MOVIE                                      &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & MIT-RESTAURANT                                 &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & MetaLWOz                                       & 37884                        &                           &                           & N/A                       \\ \cline{2-6} 
%                                                & STAR                                           & 5,820                        &                           & 20\%                      & KB                        \\ \cline{2-6} 
%                                                & SalesBot                                       & 2,014 +1902                  &                           &                           &                           \\ \cline{2-6} 
%                                                & KETOD                                          & 4247                         & 545                       & 532                       &                           \\ \cline{2-6} 
%                                                & CraigslistBargains                             &                              &                           &                           & KB                        \\ \cline{2-6} 
%                                                & MS-DC                                          &                              &                           &                           & KB                        \\ \cline{2-6} 
%                                                & CamRest676 (A subset of MultiWOZ training set) & 680                          &                           &                           &                           \\ \cline{2-6} 
%                                                & CaSiNo                                         &                              &                           &                           & KB                        \\ \cline{2-6} 
%                                                & ABCD                                           & 8034                         &                           &                           &                           \\ \cline{2-6} 
%                                                & Task2Dial                                      &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & HDSA-Dialog                                    &                              &                           &                           &                           \\ \cline{1-6} 
% \textbf{Single Turn}                           & E2E                                            & 4,862 & 547 & 630  & N                         \\ \cline{1-6} 
% \multirow{3}{*}{\textbf{Dialogue Rewrite}}     & GECOR                                          &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & CANARD                                         & 40,527                       &                           &                           & N                         \\ \cline{2-6} 
%                                                & MuDoCo                                         & 8,429                        &                           &                           & N                         \\ \cline{1-6} 
% \multirow{13}{*}{\textbf{Dialog Summarization}} & TweetSumm                                      &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & SAMSum                                         &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & DialogSum                                      &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & AMI                                            &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & ICSI                                           &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & QMSum                                          &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & MediaSum                                       &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & SummScreen-ForeverDreaming                     &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & SummScreen-TVMegaSite                          &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & ConvoSumm                                      &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & CRD3 (Need Processing)                         &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & ECTSum (Need processing)                       &                              &                           &                           &                           \\ \cline{2-6} 
%                                                & EmailSum (Need Processing)                     &                              &                           &                           &                           \\ \cline{1-6} 
% \end{tabular}
% \caption{Statistics of the DialogStudio Collections.}
% \label{tab:data}
% \end{table}

\subsubsection{Dialog Processing}

% \subsubsection{format}
\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{Tex/Figs/format.png}
\caption{Dialog Format} 
\label{fig:format}
\end{figure}
% general
For each dialog, we transfer it into the format shown in Fig.~\ref{fig:format}. The file store each dialog in a dictionary. The key of each dialog consists of the dataset name, split set (train/val/test), and index number in terms of a number. The value of each dialog has its "original dialog id", "original dialog info" which contains all dialog-level annotation, and "log", containing all dialog turns as a list. The value also contains "external knowledge", which is described in the following section (Sec.~\ref{sec:ek}). For each dialog turn, we conclude six main parts: "turn id", "user utterance", "system utterance", "dialog history", "original user side information", and "original system side information".

% speaker
In our collection of datasets, not all dialogs take place in the scenario between a "user" and a "system". Some happen between two Amazon Mechanical Turk (AMT) agents, or labeled as "customer" and "agent". For easier data loading and post-processing, we uniform all speaker who seeks help with the task as the "user" and the other speaker who helps solve the task as the "system". For a negotiation or bargain task like CaSiNo or CraigslistBargains, we consider whoever starts the conversation as the "user". For some multi-party dialog datasets, e.g. AMI and ICSI, please refer to Appendix~\ref{sec:appendix_tod} for a more detailed explanation.


% turn
Different dialog dataset has a different strategy to define a turn. Some consider an utterance from any speaker to be a single turn, while some combine a pair of utterances from both speaker sides as a turn. To be consistent across all datasets, we consider each turn contains utterances and annotations from both the user side and the system side. As shown in Fig.~\ref{fig:format}, we have a list of turns under "log" as a result.

% utt (consecutive, ignore the first utterance)
Since some datasets originally consider each utterance as a single turn, there exist cases where multiple consecutive turns contain utterances from the same side. To transfer these turns into our format, we concatenate these utterances together as a single long utterance, as well as combine the turn-level annotations of these turns. 
There are also cases that the system side initializes the conversation with a welcoming sentence, e.g. "Hello, how can I help you today?" Usually, these starting sentences from the system side have low diversity and can be easily replaced with templates if needed. Furthermore, we focus more on how to generate responses to user utterances. Therefore, we skip these initial utterances from the system side and consider the user side starting the conversation by default.

% other annotation
Since different datasets focus on different tasks, they have various annotations for both turn-level and dialog-level. Instead of focusing on each of these auxiliary tasks, we care more about the response generation and general task-oriented tasks, e.g. dialog state tracking. Therefore, we conclude all these dialog-level annotations into a dictionary "original dialog info" and turn-level annotation into dictionaries called "original user/system side information" correspondingly. We do not simply remove this information in case the user of our DialogStudio collection is interested in these auxiliary tasks. As for the annotation used for our pre-training tasks, we will describe it in more detail in the following Sec.~\ref{sec:ek}.

\subsubsection{External Knowledge}\label{sec:ek}
In our pre-training with task-oriented dialogs, we consider only three dialog tasks: response generation, dialog state tracking, and intent classification. Since each dialog dataset focuses on specific tasks or domains and has a different database, as well as an annotation schema, we propose to insert this knowledge into the input sequence, as a dependency for the model's generation.

\noindent\textbf{Response Generation}
% As shown in Fig.~\ref{fig:format}, we reformat all dialogs utterances into a list of turns. Each turn includes utterances from both the system and user sides. 
% % user starts
% We assume the user side always starts the conversation. If the system give an introducing sentence in the original data, e.g. "hello, how can I help you today?", we simply ignore this sentence.
% % continue user or system turn in original 
% There are also some consecutive turns of only single-side utterances. We consider them as one single turn in our format and concatenate these utterances together.
% \begin{itemize}
%     \item candidate result number
%     \item must include used one; others random sample
% \end{itemize}
Unlike MultiWOZ~\citep{multiwoz2018}, most of the datasets do not contain delexicalized system responses, which replace task-related key tokens with a placeholder, e.g. "The address of the hotel is [hotel-address]." However, a considerable part of the system responses contains external knowledge, e.g. database. To make the generation training more reasonable, we propose to include related external knowledge into the input sequence. For example, if the user is looking for a hotel and asking for its address. And the system response is based on the database searched hotel results. However, during the training, the model does not have access to the database. Therefore, we insert the information of the resulting hotel into the input sequence. To simulate the realistic situation and avoid directly providing the model with the ground truth resulting hotel, we also randomly sample four other candidate results and mix them with the ground truth result. All information about these five results is converted into a string and inserted into the input sequence.  

\noindent\textbf{Dialog State Tracking}
Since each dataset has a specific annotation schema, it is not reasonable to require the model to generate the designed dialog states without knowing the schema in ahead. Therefore, we propose to insert the schema into the input sequence. For datasets like SGD~\citep{rastogi2020towards}, which already provides annotation schema, we directly convert the dictionary-structured schema into a string. For the rest that does not have a schema file, we loop over all dialog and collect the dialog state annotation to form up a schema. We provide not only the domain, and slot type but also the slot value in the schema string. For those categorized dialog slots like "hotel star-ratings", which have a fixed number of candidate values, we provide all possible values. For others that have unlimited possible values, e.g. "stay night", we randomly sample ten values, in order to teach the model what slot values look like corresponding to these slot types.

\noindent\textbf{Intent Classification}
Similar to the dialog state tracking task, the annotation scheme for dialog intents is designed in different ways for different dialog datasets. Therefore, we extract the schema directly from schema file if it exists. As for the dataset that there is no schema, we loop over all dialogs in the dataset to collect all possible intents. 

Not all datasets provide detailed annotation for dialog states, intents, or even databases. For dialog state tracking and intent classification tasks, we select only dialogs with corresponding annotations for training. Since all data is used for response generation, we leave the external knowledge value for the database blank if there is no related database.

% \subsection{Conversational Recommendation}
% \subsection{Dialogue Understanding}
% \subsection{Dialogue Summarization}

==> Tex/evaluation.tex <==
\section{Evaluation Metrics} \label{sec:eval}
In this section, we present the methodologies and metrics used to assess the performance of our DialogOhama model. The evaluation process aims to measure the model's ability to both solve task-oriented dialogs and understand general prompt-based instruction. We employ a combination of quantitative benchmarks, qualitative analysis, and real-world applications to provide a comprehensive assessment of our model.

\textcolor{red}{Evaluation metrics}
BLEU-4, ROUGE-L, BERTSCORE, CHRF, CHATGPT

\textcolor{red}{Setting}
zero-shot and few-shot

\textcolor{red}{Alphaca}
FAST-T5-instruct

\subsection{Evaluation for Dialog Skills}
\noindent\textbf{Evaluation from GODEL}


GODEL~\citep{peng2022godel} provides a benchmark to evaluate model's ability for task-oriented dialogs and knowledge grounding.

\paragraph{COQA} 
COQA~\citep{reddy2019coqa} is a multi-turn conversational question answering dataset that contains 127,000 questions with answers collected from more than 8000 conversations. Each conversation is collected by pairing two crowdworkers to chat about a passage in the form of conversational questions and answers. 

\textbf{Wizard of Wikipedia}
is a dataset of multi-turn knowledge grounded di- alogs between an apprentice and a wizard, who has access to Wikipedia sentences and labels the sentences utilized for each utterance they made. To focus on grounded response generation, we use the gold Wikipedia sentences provided at each turn of the dialog.

\textbf{Wizard of Internet}
is an open-domain dialog dataset grounded on internet retrieved sentences. At each turn, the wizard can issue a free text web search and replies to the ap- prentice grounding the response on the retrieved sentences. Similarly, we use the gold retrieved sentences provided at each turn of the dialog.

\textbf{MultiWOZ 2.2}
is a multi-domain task-oriented dialog dataset that contains 8438/1000/1000 dialogs for train- ing/validation/testing, respectively. Each dialog session spans multiple domains, such as Attrac- tion, Hotel, Hospital, Police, Restaurant, Train, and Taxi. This dataset is challenging owing to its multi-domain setting and diverse language styles. For this dataset, we consider the task of context- to-response

We focus on zero-shot or one-shot evaluation.

\begin{table*}[]
\resizebox{1.0\linewidth}{!}{
\centering
\begin{tabular}{l|cccccc}
\hline
                   & \multicolumn{2}{c}{Wizard of Internet}  & \multicolumn{2}{c}{Wizard of Wikipedia} & \multicolumn{2}{c}{CoQA} \\ \hline
                   & RougeL & \multicolumn{1}{c|}{BERTScore} & RougeL & \multicolumn{1}{c|}{BERTScore} & RougeL    & BERTScore    \\ \hline
FlanT5-large       & 7.91   & \multicolumn{1}{c|}{37.33}     & 6.51   & \multicolumn{1}{c|}{34.2}      & 6.76      & 38.42        \\
GODEL-large        & 14.56  & \multicolumn{1}{c|}{44.93}     & 22.51  & \multicolumn{1}{c|}{51.07}     & 48.58     & 64.09        \\ \hline
FlanT5-base        & 10.92  & \multicolumn{1}{c|}{40.82}     & 10.20  & \multicolumn{1}{c|}{39.01}     & 7.02      & 37.59        \\
GODEL-base         & 11.56  & \multicolumn{1}{c|}{41.47}     & 24.49  & \multicolumn{1}{c|}{51.74}     & 8.27      & 34.93        \\
DialogDolphin-base & 13.26  & \multicolumn{1}{c|}{45.14}     & 15.29  & \multicolumn{1}{c|}{45.86}     & 30.31     & 50.14        \\ \hline
\end{tabular}}\caption{Zero-shot results on test sets of Wizard of Internet, Wizard of Wikipedia, and CoQA.}
\end{table*}
% \noindent\textbf{Evaluation on Super-NaturalInstructions
% }
\begin{table}[]
\begin{tabular}{l|cccc}
\hline
                   & \multicolumn{2}{c}{}                    & \multicolumn{2}{c}{}                    \\ \hline
                   & RougeL & \multicolumn{1}{c|}{BERTScore} & ChatGPT & \multicolumn{1}{c|}{Naturall} \\ \hline
FlanT5-large       &        & \multicolumn{1}{c|}{}          &         & \multicolumn{1}{c|}{}         \\
GODEL-large        &        & \multicolumn{1}{c|}{}          &         & \multicolumn{1}{c|}{}         \\
GODEL-base         &        & \multicolumn{1}{c|}{}          &         & \multicolumn{1}{c|}{}         \\
DialogDolphin-base &        & \multicolumn{1}{c|}{}          &         & \multicolumn{1}{c|}{}         \\ \hline
\end{tabular}\caption{multiwox}
\end{table}

\subsection{Evaluation on Super-NaturalInstructions
}

\cite{wang2022super} introduces the Super-NaturalInstructions benchmark on more than 1600 tasks. We select 3 categories with 44 tasks from the held-out test set, i.e., Coreference Resolution, Dialogue Act Recognition and Textual Entailment. . The tasks are both relevant to dialog evaluation, and all the evaluation tasks and datasets are unseen in the training time.

Specifically, we follow all settings in \cite{wang2022super} and fine-tune DialogOhana on the 756 training tasks, each task with 100 examples and we fine-tune it for 3 epochs.  

\textcolor{red}{Will put a table here to compare and analyze with OPT-IML, GODEL, DialogOhana}

\begin{table*}[]
\resizebox{1.0\linewidth}{!}{
\centering
\begin{tabular}{l|ccc|cc}
\hline
                 & \begin{tabular}[c]{@{}c@{}}Coreference Resolution \\ (14 tasks)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dialogue Act Recognition \\ (7 tasks)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Textual Entailment \\ (27 tasks)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Average\\ (48 tasks)\end{tabular}           & \begin{tabular}[c]{@{}c@{}} Average \\ (all 154 tasks)\end{tabular}\\ \hline
OPT 30B          & 21.3/1.1                          & 35.2/4.1                           & 40.3/0.9                      & 32.3/2.0           & -                                           \\
OPT-IML 30B      & 37.4/41.6                         & 51.4/51.8                          & 54.7/47.8                     & 47.9/47.1          & -                                           \\
OPT 175B         & 21.0/4.2                          & 37.1/16.8                          & 41.6/2.2                      & 33.3/7.7           & -                                           \\
OPT-IML 175B     & 39.0/49.8                         & 61.2/60.2                          & 54.3/51.0                     & 51.5/53.6          & -                                           \\ \hline
TK-Instruct 3B   & 38.7/44.9                            & 45.7/53.0                             & 48.8/46.0                        & 44.4/48.0             & 43.0/54.33                                     \\
TK-Instruct 11B  & 32.3/62.3                         & 51.1/69.6                          & 55.0/64.1                     & 46.1/65.3          & 46.1/60.07                                  \\
DialogDolphin 3B & 41.3/63.2                         & 57.5/64.1                          & 52.3/58.7                     & \textbf{50.4/62.0} & \textbf{46.3/58.24}                         \\ \hline
\end{tabular}}\caption{0-shot/2-shot RougeL evaluation on unseen datasets and unseen tasks. }
\end{table*}

\subsection{Evaluation for General Understanding}
% MMLU

\subsection{Evaluation for General Generation}
% 

% Datasets
% GODEL: Four datasets (CoQA, WOW, WOI, MultiWOZ)
% In-context MultiWOZ DST
% OPT-IML: 44 Tasks (coreference resolution, dialog act recognition, text entailment)
% Intent detection (Add later)

%MMLU 


==> Tex/experiment.tex <==
\section{Experiment Details}
In this section, we introduce more details about how we conduct our pre-training.

\subsection{Three-Stage Training Strategy}
We divide our training process into three states.
\begin{itemize}
    \item \textbf{Dialog Pre-training}
    In the first stage, we mainly mix 18 task-oriented dialog (ToD) datasets, 2 conversational recommendation datasets, 2 dialog safety datasets and one chitchat dataset, which is SODA~\citep{kim2022soda}. 
    % There are in total one million ToD dialogs and one million chitchat dialogs. To balance data from these domains, we sample $10\%$ of the data from the ToD datasets and $10\%$ of the chitchat. 
    To enhance the model's robustness, we also sample $20\%$ of the used ToD data and change the order of "Instruction", "External Knowledge", and "Dialog Input". This introduces more variety in the input format. With 0.8 million new examples, this will further help the model adapt to different input structures.
    We also introduce an additional task by sampling another $10\%$ of data from the ToD datasets and let the model generate dialog history based on the system response and external knowledge. This can potentially improve the model's understanding of the relationship between the dialog history, system response, and external knowledge.
    \item \textbf{Prompt Tuning}
    Following \cite{longpre2023flan} work, we sample ten million data examples from FLAN-Collection for prompting tuning. 
    The original FLAN-Collection contains data from T0, FLAN-v1, NIV2, and Chain-of-Thought.
    To enhance the model's ability for both zero-shot and few-shot learning, we also mix zero-shot and few-shot examples half-half. The number of examples in the few-shot setting ranges from one to 10 randomly.
    In order to avoid the forgetting problem, we also mix 20$\%$ dialog data into this training stage.
    \item \textbf{Knowledge-grounded Training}
    Most of the task-oriented dialogs, as well as conversational recommendations; knowledge grounded QA, etc., involve information retrieval from an external knowledge base. Traditional methods generate a query or multiple keywords for searching the external knowledge base. We propose to train our model in an end-to-end way. For each dialog during the training, we transfer the corresponding external knowledge into a string and include the string in the input sequence. We also ask the model to generate a dialog response based on the external knowledge in the prompt.
\end{itemize}






==> Tex/neurips_requestments.tex <==
\section{NeurIPS requirements}
Next to a scientific paper, authors must also submit supplementary materials which provide full detail on how the data was collected and organized, what kind of information it contains, how it should be used ethically and responsibly, as well as how it will be made available and maintained. 

Authors are free in describing this to the best of their ability. For instance, dataset papers could make use of dataset documentation frameworks, such as datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks. For benchmarks, best practices on reproducibility should be followed.

As part of this track, we aim to gather advice on best practices in constructing, documenting, and using datasets, including examples of known exemplary as well as problematic datasets, and create a website that makes this information easily accessible.



==> Tex/related_works.tex <==
\section{Related Works}\label{sec:relate}
\subsection{Instruction Finetuning}
\subsection{Dataset Collection}
InstructDial, UnifiedSKG, NIV2, Flan, T0

==> conclusion.tex <==
\section{Conclusion}
In this paper, we improve the performance of few-shot intent detection via contrastive pre-training and fine-tuning. It first conducts self-supervised contrastive pre-training on collected intent detection datasets without using any labels, where the model implicitly learns to separate fine-grained intents. Then it performs the few-shot fine-tuning based on the joint intent classification loss and supervised contrastive learning loss, where the supervised contrastive loss encourages the model to  distinguish intents explicitly. Experimental results on three challenging datasets show that our proposed method achieves state-of-the-art performance.




==> experiments.tex <==

\begin{table*}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\hline
                                                                  & \multicolumn{2}{c|}{CLINC150} & \multicolumn{2}{c|}{BANKING77} & \multicolumn{2}{c}{HWU64} \\
Model                                                             & 5-shot        & 10-shot       & 5-shot        & 10-shot       & 5-shot      & 10-shot      \\ \hline
CPFT                                                              & 92.34         & 94.18         & 80.86         & 87.20          & 82.03       & 87.13        \\ \hdashline
w/o Contrastive pre-training                                       & -4.15         & -2.63         & -4.11         & -2.37         & -6.01       & -4.17        \\
w/o Supervised contrastive learning                               & -0.56         & -0.32         & -2.06         & -0.88         & -1.14       & -0.27      \\
w/o Contrastive pre-training + w/o Supervised contrastive learning & -4.35         & -2.69         & -6.82         & -2.93         & -6.47       & -4.23        
  \\ \hline
\end{tabular}} \caption{Testing accuracy ($\times 100\%$) of CPFT with variants on three datasets under 5-shot and 10-shot settings.}\label{table:ablation-study}
% \vspace{-1em}
% \vspace{-5mm}
\end{table*}

\section{Experimental Results}


 We show  the overall comparisons on three datasets in Table \ref{table:main-results}. The proposed CPFT method achieves the best performance across all datasets under both the 5-shot and 10-shot settings. Specifically,  CPFT outperforms DNNC by 1.32\% and 1.57\% on CLINC150 and HWU64 under the 5-shot setting, respectively. It also improves DNNC by 2.41\% on HWU64 under the 10-shot setting. 
 Our variances are also lower when compared with DNNC: Ours vs. DNNC: 0.39 vs. 0.57 and 0.18 vs. 0.42 on CLINC150; 0.20 vs. 0.88 and 0.48 vs. 0.21 on BANKING77; 0.51 vs. 1.00 and 0.25 vs. 0.38 on HWU64 under 5-shot and 10-shot settings, respectively.
 The improvements indicate that our proposed method has a better ability to discriminate semantically similar intents than the strong discriminate nearest-neighbor model with data augmentation.
Moreover, the DNNC training is expensive, as when training models on a single NVIDIA Tesla V100 GPU with 32GB memory, DNNC takes more than $3$ hours for 10-shot learning on CLINC150, and it needs to retrain the model for every new setting. CPFT only needs $2.5$ hours for one-time pre-training, and the  fine-tuning only takes five minutes for each new setting.  
Compared with CONVBERT+MLM, which does a self-supervised pre-training with MLM on the intent detection datasets, CPFT improves the performance by 1.43\%, 3.21\%, and 2.61\% on CLINC150, BANKING77, and HWU64 under 10-shot setting, respectively. CPFL also outperforms CONVBERT+Combined, which further adds examples-driven training and specific transformer attention design. We contribute the performance improvements to contrastive learning, which help the model discriminate semantically similar intents. 



\section{Ablation Study and Analysis}
\paragraph{Is the schema with both stages necessary?}
We conduct ablation study to investigate the effects of self-supervised contrastive pre-training and supervised contrastive fine-tuning. Table \ref{table:ablation-study} shows the testing results of CPFT with model variants on three datasets. Experimental results indicate that both stages are necessary to achieve the best performance. The self-supervised contrastive pre-training on the first stage is essential as the performance drops significantly on all datasets. We hypothesize that contrastive pre-training on the intent datasets without using labels benefits the discrimination of semantically similar utterances. Additionally, the performance also drops if without supervised contrastive learning during the few-shot fine-tuning stage. Specifically, it drops by 2\%  on BANKING77 under the 5-shot setting; the reason is that BANKING77 is a single domain dataset with many similar intents, where supervised contrastive learning can explicitly discriminate semantically similar intents with very limited training examples. 
We also jointly train the first and second stages together, and compared with the proposed CPFT schema, we observe minimal improvements. The joint training is also costly as it requires retraining the model every time for new settings. 

\paragraph{Is contrastive pre-training beneficial to the target intent dataset? }
Additionally, we study whether contrastive pre-training can benefit the intent detection when excluding the target datasets. Specifically, we pre-train the model on the datasets except for the HWU64 dataset on the first stage and do few-shot learning on HWU64 during the second stage. Compared to the model without contrastive pre-training on the first stage, the performances are improved by 1.98\% and 1.21\% under 5-shot and 10-shot settings, respectively. The improvements indicate that the contrastive pre-training is helpful to transfer knowledge to new datasets. However, there are still performance drops compared to the contrastive pre-training, including the HWU64 dataset. Which shows that it is beneficial to include the target dataset during self-supervised contrastive learning. We leave whether self-supervised contrastive pre-training only on the target intent dataset benefits as a future study.

\paragraph{Is the training sensitive to hyper-parameters?}

We also study the effects of hyper-parameters of contrastive learning, \textit{i.e.}, the  temperature $\tau$ and weight $\lambda'$. We set $\tau \,{\in}\, \{0.05,0.1,0.3,0.5\}$ and $\lambda' \,{\in}\, \{0.01,0.03,0.05, 0.1\}$. In our primary experiments, we do not find $\tau$ has a notable influence during the self-supervised contrastive pre-training on the first stage.  Besides, we found that a batch size larger than 32 works well in the pre-training phase.
% as the model implicitly learn to discriminate semantically similar utterances without using labels. 
However, during the few-shot fine-tuning stage, when setting $\tau$ to a small value $0.05$, which heavily enforces the penalty to hard negative examples and $\lambda'$ to a large value $0.1$, which increases the weight of supervised contrastive learning loss, the performance drops significantly. In addition, the batch size  influences performance on this stage. Therefore, few-shot supervised contrastive loss is sensitive to hyper-parameters
% on the second stage performs more like a regularization loss 
when there are limited training examples. 
% We leave more studies to future work.

% Jianguo Zhang, Kazuma Hashimoto, Wenhao Liu, Chien-Sheng Wu, Yao Wan, S Yu Philip, Richard Socher, and Caiming Xiong. 2020. Discriminative nearest neighbor few-shot intent detection by transferring natural language inference. In Proceed- ings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP), pages 5064–5082.

% Shikib Mehri, Mihail Eric, and Dilek Hakkani-Tur. 2020b. Example-driven intent prediction with observers. arXiv preprint arXiv:2010.08684.

% Congying Xia, Chenwei Zhang, Hoang Nguyen, Jiawei Zhang, and Philip Yu. 2020. Cg-bert: Conditional text generation with bert for generalized few-shot in- tent detection. arXiv preprint arXiv:2004.01881.

% Baolin Peng, Chenguang Zhu, Michael Zeng, and Jianfeng Gao. 2020. Data augmentation for spoken language understanding via pretrained language models. arXiv preprint arXiv:2004.13952.

% Diederik P Kingma and Max Welling. 2013. Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114.

% Alec Radford, Jong Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, et al. 2021. Learning transferable visual models from natural language supervision. Image, 2:T2.

% Inigo Casanueva, Tadas Temcinas, Daniela Gerz, Matthew Henderson, and Ivan Vulic. 2020. Efficient intent detection with dual sentence encoders. ACL 2020, page 38.

% Shikib Mehri, Mihail Eric, and Dilek Hakkani-Tur. 2020a. Dialoglue: A natural language understanding benchmark for task-oriented dialogue. preprint arXiv:2009.13570.

% Stefan Larson, Anish Mahendran, Joseph J. Peper, Christopher Clarke, Andrew Lee, Parker Hill, Jonathan K. Kummerfeld, Kevin Leach, Michael A. Laurenzano, Lingjia Tang, and Jason Mars. 2019. An Evaluation Dataset for Intent Classification and Out-of-Scope Prediction. In EMNLP, pages 1311– 1316.

==> introduction-new.tex <==
\section{Introduction}

Intent detection, aiming to identify intents from user utterances, is a key component in task-oriented dialog systems. In real systems such as Amazon Alexa, correctly identifying user intents is crucial for downstream tasks~\citep{zhang2020find,ham2020end}.  A practical challenge is data scarcity as it is expensive to annotate enough examples for emerging intents, and how to accurately identify intents in few-shot learning has raised attention.

Existing methods address the few-shot intent detection tasks mainly from two perspectives: (1) data augmentation and (2) task-adaptive training with pre-trained models. For the first category, \newcite{zhang2020discriminative} and \newcite{mehri2020example}  propose a nearest neighbor classification schema with full use of the limited training examples in both training and inference stages. 
% However, the model training is very expensive and hard to scale to tasks with several intents. 
% \citep{eda} proposes simple text editing rules such as insert and swap, and \citep{deng2019low} proposes back translation for data augmentation, while such methods have been shown not to work well on few-shot intent detection. 
\newcite{xia2020cg} and \newcite{peng2020data} propose to generate utterances for emerging intents based on variational autoencoder~\citep{kingma2013auto} and GPT-2~\citep{radford2019language}, respectively. 
% However, the generated utterances are noisy and require human filtering. 
For the second category,  \newcite{efficient_intent}  and \newcite{mehri2020dialoglue} conduct intent detection by leveraging related conversational pre-training models based on a few hundred million conversations.  Meanwhile, they devise a task-adaptive training schema where the model is pre-trained on all relative intent datasets or the target intent datasets with mask language modeling. 


However, previous methods such as data augmentation related models~\cite{liu2021augmenting} are inefficient for training and hard to scale to tasks with lots of intents. Moreover, these models do not tackle well the following scenarios: In real scenarios, the few-shot intent detection could be more challenging when there exist many fine-grained intents, especially semantically similar intents. For instance, BANKING77~\citep{efficient_intent} has a single domain with 77 intents, and CLINC150~\citep{oos-intent} has ten domains with 150 intents. 
Many intents in the datasets are similar. Therefore, training models is rather challenging when there are only limited examples. 

Inspired by the recent success of contrastive learning~\citep{he2020momentum,gunel2020supervised,chen2020simple,radford2learning,liu2021fast,gao2021simcse,liu2021contrastive}, which aims to enhance 
discrimination abilities of models,
% enforce examples from the same class close and the examples from different classes apart,
this work proposes improving few-shot intent detection via Contrastive Pre-training and Fine-Tuning (CPFT). Intuitively, we first learn to implicitly discriminate semantically similar utterances via contrastive self-supervised pre-training on intent datasets without using any intent labels. 
We then jointly perform few-shot intent detection and supervised contrastive learning. The supervised contrastive learning helps the model explicitly learn to pull utterances from the same intent close and push utterances across different intents apart. 

% We also notice some very recent works~\citep{liu2021fast,gao2021simcse,gunel2020supervised} adopting contrastive learning in natural language processing tasks. Our work differs them in: Firstly, we specifically tackle the few-shot intent detection task; Secondly, we employ contrastive  learning in both self-supervised pre-training and supervised fine-tuning stages.
% with two stages. 
% rather than general \textcolor{red}{single-stage contrastive pre-training or fine-tuning}. 
% We also do not need to specifically design and handle hard negative examples.

Our contributions are summarized as follows: 1) We design a simple yet effective few-shot intent detection schema via contrastive pre-training and fine-tuning. 2) Experimental results verify the state-of-the-art performance of CPFT on three challenging datasets under 5-shot and 10-shot settings.

==> introduction.tex <==
\section{Introduction}

First, we unify the dialog into unified format

Instruction:
Your task is to generate a dialog belief state based on a given dialog context and structured belief state. The structured belief state presents candidate values for different slots. For example, 'hotel-pricerange' may have values like 'cheap', 'dontcare', 'expensive', 'moderate'. If a slot has unlimited potential values, its default value in the structured belief state will be 'none' (e.g., 'hotel-name: none'), and you are required to find the actual value from the dialog context. For slots that are either not mentioned or irrelevant to the dialog, assign them the value 'none'. The generated dialog belief state should be in the format 'slot-name: value'. Maintain the order of the slots as per the structured belief state.

Structured belief state:
hotel-pricerange: cheap, dontcare, expensive, moderate; hotel-type: guesthouse, hotel; hotel-parking: dontcare, free, no, yes; hotel-book day: friday, monday, saturday, sunday, thursday, tuesday, wednesday; hotel-book people: 1, 2, 3, 4, 5, 6, 7, 8; hotel-book stay: 1, 2, 3, 4, 5, 6, 7, 8; hotel-area: centre, dontcare, east, north, south, west; hotel-stars: 0, 1, 2, 3, 4, 5, dontcare; hotel-internet: dontcare, no, yes; hotel-name: none; train-destination: none; train-day: dontcare, friday, monday, saturday, sunday, thursday, tuesday, wednesday; train-departure: none; train-arriveby: none; train-book people: 0, 1, 10, 15, 2, 3, 4, 5, 6, 7, 8, 9; taxi-destination: none; taxi-departure: none; taxi-leaveat: none; train-leaveat: none; attraction-area: cambridge, centre, dontcare, east, north, south, west; restaurant-pricerange: cheap, dontcare, expensive, moderate; restaurant-area: centre, east, north, south, west; restaurant-food: none; attraction-name: none; restaurant-name: none; attraction-type: architecture, boat, church, cinema, college, concerthall, entertainment, hotspot, multiple sports, museum, nightclub, park, special, swimmingpool, theatre; restaurant-book day: friday, monday, saturday, sunday, thursday, tuesday, wednesday; restaurant-book people: 1, 2, 3, 4, 5, 6, 7, 8; restaurant-book time: none; taxi-arriveby: none

Dialog context:
<USER> hi , i am looking for a train that is going to cambridge and arriving there by 20:45 , is there anything like that ? <SYSTEM> there are over 1,000 trains like that . where will you be departing from ? <USER> i am departing from birmingham new street . <SYSTEM> can you confirm your desired travel day ? <USER> i would like to leave on wednesday <SYSTEM> i show a train leaving birmingham new street at 17:40 and arriving at 20:23 on wednesday . will this work for you ? <USER> that will , yes . please make a booking for 5 people please . <SYSTEM> i have booked your train tickets , and your reference number is a9nhso9y . <USER> thanks so much . i would also need a place to say . i am looking for something with 4 stars and has free wifi . <SYSTEM> how about the cambridge belfry ? it has all the attributes you requested and a great name ! maybe even a real belfry ? <USER> that sounds great , could you make a booking for me please ? <SYSTEM> what day would you like your booking for ? <USER> please book it for wednesday for 5 people and 5 nights , please .

Generated belief state:


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
\usepackage{amsmath,amsfonts,bm,amsthm,amssymb,mathrsfs,algorithm,algorithmic,url,xcolor}
\usepackage{booktabs,enumitem,multicol,caption,subcaption,pifont,tikz,listings,wrapfig,lipsum,circledsteps,arydshln,hyperref,multirow}
\usepackage{relsize,footnote,makecell}


\hypersetup{
    colorlinks,
    linkcolor={blue!50!black},
    citecolor={blue!50!black},
    urlcolor={red!50!black}
}

\lstset{
    language=Python,
    numberstyle=\tiny,
    mathescape=true, 
    language=Python, 
    columns=fullflexible,
    flexiblecolumns=true,
}

\newcommand{\circled}[1]{\textcircled{\raisebox{-0.9pt}{#1}}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem} %[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{theorem*}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{fact}{Fact}
\newtheorem{conjecture}{Conjecture}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vpsi{{\bm{\psi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}





% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\def\ps{\pmb{s}}
\def\ph{\pmb{h}}
\def\pa{\pmb{a}}
\def\po{\pmb{o}}
\def\pg{\pmb{g}}

\newcommand{\abs}[1]{\left\vert#1\right\rvert}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\br}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\given}{\,|\,}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\denv}{\gD_{\mathrm{env}}}
\newcommand{\dmodel}{\gD_{\mathrm{model}}}


\newcommand{\dbtrue}{d_{\pi_b}^{P^{*}}}
\newcommand{\dpitrue}{d_{\pi}^{P^{*}}}
\newcommand{\dbfake}{d_{\pi_b}^{\widehat{P}}}
\newcommand{\dpifake}{d_{\pi}^{\widehat{P}}}

\newcommand{\dbgtrue}{d_{\pi_b,\gamma}^{P^{*}}}
\newcommand{\dpigtrue}{d_{\pi,\gamma}^{P^{*}}}
\newcommand{\dbgfake}{d_{\pi_b,\gamma}^{\widehat{P}}}
\newcommand{\dpigfake}{d_{\pi,\gamma}^{\widehat{P}}}
\newcommand{\rmax}{r_{\max}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}

\newcommand{\wQ}{{\widehat{Q}}}
\newcommand{\wP}{{\widehat{P}}}
\newcommand{\trueP}{{P^{*}}}

\newcommand*{\defeq}{\stackrel{\mathsmaller{\mathsf{def}}}{=}}

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\wrt}{\textit{w.r.t.}}
\newcommand{\etc}{\textit{etc.}}
\newcommand{\myparagraph}[1]{\textbf{#1~~}}

\newcommand{\rulesep}{\unskip\ \vrule\ }

\newcommand{\bad}[1]{\hfill \color{Maroon}//~#1}
\newcommand{\good}[1]{\hfill \color{SeaGreen}//~#1}

\newcommand{\rewardnet}{\texttt{RewardNet}~}

\newcommand{\rewardNet}{\texttt{RewardNet}~}

\newcommand{\rewardMLE}{\texttt{RewardMLE}~}

\newcommand{\rewardmle}{\texttt{RewardMLE}~}

==> methodology.tex <==
% \section{Task Definition for Few-Shot Intent Detection}



\section{CPFT Methodology}

We consider a few-shot intent detection task that handles $C$
% $\mathcal{C}\,{=}\,\{C_1, C_2, \ldots, C_N\}$ 
user intents, where the task is to classify a user utterance $u$ into one of the $C$ classes.
We set balanced K-shot learning for each intent~\cite{zhang2020discriminative,efficient_intent}, i.e., each intent only includes $K$ examples in the training data. As such, there are in total $C\cdot K$ training examples.  

In the following section, we first describe the self-supervised contrastive pre-training for utterance understanding before introducing the supervised fine-tuning for few-shot intent detection.

\subsection{Self-supervised Pre-training}
We retrieve the feature representation $\mathbf{h}_i$ for the $i$-th user utterance through an encoder model, which in this paper is BERT~\cite{bert}, \textit{i.e.}, $\mathbf{h}_i=\text{BERT}(u_i)$. 
We implicitly learn the sentence-level utterance understanding and discriminate semantically similar utterances through the self-supervised contrastive learning method~\citep{wu2020clear,liu2021fast,gao2021simcse}:
% \vspace{-0.04in}
\begin{equation}
    \label{eq:stage-1-unsupvised cl}
    \small
    \mathcal{L}_{\text{uns\_{cl}}}=-\frac{1}{N}\sum_{i=1}^{N}\log\frac{\exp(\text{sim}(\mathbf{h}_i,\bar{\mathbf{h}}_i)/\tau)}{\sum_{j=1}^{N}\exp(\text{sim}(\mathbf{h}_i,\bar{\mathbf{h}}_j)/\tau)},
\end{equation}
where $N$ is the number of sentences in a batch. $\tau$ is a temperature parameter that controls the penalty to negative samples. $sim(\mathbf{h}_i,\bar{\mathbf{h}_i})$ denotes the cosine similarity between two input vectors $\mathbf{h}_i$ and $\bar{\mathbf{h}_i}$.  $\bar{\mathbf{h}_i}$ represents the representation of sentence $\bar{u_i}$, where $\bar{u_i}$ is from the same sentence $u_i$ but few (10\%) tokens are randomly masked~\cite{bert}. Specifically,  we dynamically mask tokens during batch training~\citep{tod-bert}, i.e., a sentence has different masked positions across different training epochs, and we find it is beneficial to the utterance understanding. The sentence $u_i$ and  $\bar{u_i}$ are inputted together to a single encoder during the batch training~\citep{gao2021simcse}. 

Besides the sentence-level enhancement, we also add the mask language modeling loss~\cite{bert,tod-bert} to enhance the token-level utterance understanding:
% \vspace{-0.04in}
\begin{equation}
    \label{eq:stage-1-mlm}
    \small
    \mathcal{L}_{\text{mlm}}=-\frac{1}{M}\sum_{m=1}^{M}\log P(x_m),
\end{equation}
where $P(x_m)$ denotes the predicted probability of a masked token $x_m$ over the total vocabulary, and $M$ is the number of masked tokens in each batch. 

Our total loss for each batch is $\mathcal{L}_{\text{stage1}}=\mathcal{L}_{\text{uns\_{cl}}}+\lambda\mathcal{L}_{\text{mlm}}$, where $\lambda$ is a weight hyper-parameter.

\subsection{Supervised Fine-tuning}
Through self-supervised learning in the first stage, the model efficiently utilizes many unlabeled user utterances. The model is given very limited examples in the second stage, such as 5 and 10 examples for each intent.  To better understanding user intents, especially when intents are similar to each other, we utilize a supervised contrastive learning method~\citep{gunel2020supervised} and train it together with an intent classification loss. We treat two utterances from the same class as a positive pair and the two utterances across different classes as a negative pair for contrastive learning. Unlike the previous work, the utterance and itself could also be a positive pair as we input them together to the single encoder. Their feature representations are different due to the dropout of BERT.  The corresponding loss is shown as the following:
% \vspace{-0.04in}
\begin{equation}
 \small
     \mathcal{L}_{\text{s\_{cl}}}=-\frac{1}{T}\sum_{i=1}^{N}\sum_{j=1}^{N}\mathds{1}_{y_i=y_j} \log\frac{\exp(\text{sim}(\mathbf{h}_i,\mathbf{h}_j)/\tau)}{\sum_{n=1}^{N}\exp(\text{sim}(\mathbf{h}_i,\mathbf{h}_n)/\tau)},
\end{equation}
where $T$ is the number of pairs from the same classes in the batch. 

Next is the intent classification loss:
% \vspace{-0.04in}
\begin{equation}
\small
    \mathcal{L}_{\text{intent}}=-\frac{1}{N}\sum_{j=1}^{C}\sum_{i=1}^{N}\log P(C_j|u_i),
\end{equation}
where $P(C_j|u_i)$ is the predicted probability of the $i$-th sentence to be the $j$-th intent class.

We jointly train the two losses together at each batch: $\mathcal{L}_{\text{stage2}}=\mathcal{L}_{\text{s\_{cl}}}+\lambda' \mathcal{L}_{\text{intent}}$, where $\lambda'$ is a weight hyper-parameter.




\begin{table}[]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{lccc}
\hline
\textbf{Name} & \multicolumn{1}{l}{\textbf{\# Utterance}} & \multicolumn{1}{l}{\textbf{\# Intent}} & \multicolumn{1}{l}{\textbf{\# Domain}} \\ \hline
CLINC150~\citep{oos-intent}      & 18200                                     & 150                                    & 10                                     \\
BANKING77~\citep{efficient_intent}     & 10162                                     & 77                                     & 1                                      \\
HWU64~\citep{liu2019benchmarking}         & 10030                                     & 64                                     & 21                                     \\
TOP~\citep{gupta2018semantic}           & 35741                                     & 25                                     & 2                                      \\
SNIPS~\citep{coucke2018snips}         & 9888                                      & 5                                      & -                                      \\
ATIS~\citep{tur2010left}          & 4978                                      & 21                                     & -                           \\ \hline         
\end{tabular}}\caption{Data statistics for intent detection datasets.}\label{table:data-stats}
% \vspace{-1em}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[ht]
% \small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\hline
                                     & \multicolumn{2}{c|}{CLINC150} & \multicolumn{2}{c|}{BANKING77} & \multicolumn{2}{c}{HWU64} \\
Model                                & 5-shot        & 10-shot       & 5-shot        & 10-shot       & 5-shot      & 10-shot      \\ \hline
RoBERTa+Classifier~\citep{zhang2020discriminative}                   & 87.99         & 91.55         & 74.04         & 84.27         & 75.56       & 82.90         \\
USE~\citep{efficient_intent}                                  & 87.82         & 90.85         & 76.29         & 84.23         & 77.79       & 83.75        \\
CONVERT~\citep{efficient_intent}                              & 89.22         & 92.62         & 75.32         & 83.32         & 76.95       & 82.65        \\
USE+CONVERT~\citep{efficient_intent}                          & 90.49         & 93.26         & 77.75         & 85.19         & 80.01       & 85.83        \\
CONVBERT~\citep{mehri2020dialoglue}                             & -             & 92.10         & -             & 83.63         & -           & 83.77        \\
CONVBERT + MLM~\citep{mehri2020dialoglue}                       & -             & 92.75         & -             & 83.99         & -           & 84.52        \\
CONVBERT + Combined~\citep{mehri2020example} & -             & 93.97         & -             & 85.95         & -           & 86.28        \\
DNNC~\citep{zhang2020discriminative}                                 & 91.02         & 93.76         & 80.40         & 86.71         & 80.46       & 84.72        \\ \hdashline
CPFT                                & \textbf{92.34}         & \textbf{94.18}         & \textbf{80.86}         & \textbf{87.20}          & \textbf{82.03}       & \textbf{87.13}        \\ \hline
\end{tabular}}\caption{Testing accuracy ($\times 100\%$) on three datasets under 5-shot and 10-shot settings.}\label{table:main-results}
% \vspace{-0.5em}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> related-work.tex <==
\section{Related Work}
Since this work is related to few-shot intent detection and contrastive learning, we review recent work from both areas in this section. 

The few-shot intent detection task typically includes three scenarios: (1) learn a intent detection model with only $K$ examples for each intent~\citep{zhang2020discriminative,mehri2020dialoglue,efficient_intent}; (2) given a model trained on existing intents with efficient labeled examples, learn to generalize the model to new intents with only $K$ examples for each new intent~\citep{xia2020composed,xia2020cg,xia2021pseudo};  (3) learn to identify both in-domain  and  out-of-scope queries with only $K$ examples for each intent~\citep{zhang2020discriminative,zhang2021pretrained, xia2021incremental}. 

In this work, we focus on the first scenario, and several methods have been proposed to tackle the challenge. Specifically, \newcite{zhang2020discriminative} proposes a  data augmentation schema, which pre-trains a model on annotated pairs from natural language inference (NLI) datasets and designs the nearest neighbor classification schema to adopt the transfer learning and classify user intents.  However, the training is expensive and hard to scale to tasks with hundreds of intents~\cite{liu2020basket}. \newcite{mehri2020example,efficient_intent} propose the task-adaptive training, which leverages models pre-trained from a few hundred million dialogues to tackle few-shot intent detection. It also includes an unsupervised mask language modeling loss on the target intent datasets and shows promising improvements. 


Contrastive learning has shown superior performance on various domains, such as visual representation~\citep{he2020momentum,chen2020simple,radford2learning}, graph representation~\cite{qiu2020gcc,you2020graph}, and recommender systems~\cite{liu2021contrastive}. Moreover, recent works also adopt contrastive learning in natural language processing tasks~\citep{gunel2020supervised,liu2021fast,gao2021simcse}, which employs the contrastive learning to train the encoder. Specifically, \cite{gunel2020supervised} designs a supervised contrastive learning loss for fine-tuning data. \newcite{gao2021simcse}  designs a simple contrastive learning framework through dropout and it shows state-of-the-art performance on unsupervised and full-shot supervised semantic textual similarity tasks. \newcite{liu2021fast} designs self-supervised Mirror-BERT framework with two types of data augmentation: randomly erase or mask parts of the input texts; feature level augmentation through dropout.

Our work differs from them in several respects: Firstly, we specifically tackle the few-shot intent detection task rather than the general full-shot learning; Secondly, we design a schema and employ contrastive learning in both self-supervised pre-training and supervised fine-tuning stages. 

==> settings.tex <==

\section{Experimental Settings}

\subsection{Datasets}

\paragraph{Pre-training Datasets}
We collected six public datasets consisting of different user intents. The dataset statistics are shown in Table  \ref{table:data-stats}.\footnote{\url{https://github.com/jianguoz/Few-Shot-Intent-Detection}} For fair comparisons, we exclude their test sets during the pre-training phase, which is different from previous work~\citep{mehri2020dialoglue,mehri2020example}, where they use the whole datasets. We also remove utterances with less than five tokens, and there are 80,782 training utterances in total. We conduct self-supervised pre-training on the collected utterances without using labels. 

% , and the dataset statistics are shown in Table \ref{table:data-stats}. 
% \footnote{comment: I assume Table \ref{table:data-stats} is the statistics on the raw dataset. When adding the number of utterance, the number is 88,999, which does not match 80,782 here. If True, I would suggest to refer to Table \ref{table:data-stats} at the beginning of this paragraph. "We collected six public datasets consisting of different user intents, and the dataset statistics are shown in Table \ref{table:data-stats}."}



\paragraph{Evaluation Datasets}
To better study the more challenging fine-grained few-shot intent detection problem and compare with recent state-of-the-art baselines,
we pick up three challenging intent detection datasets for evaluation, \textit{i.e.}, CLINC150~\citep{oos-intent}, BANKING77~\citep{efficient_intent} and HWU64~\citep{liu2019benchmarking}. CLINC150 contains 23,700 utterances across ten different domains, and there are in total 150 intents. BANKING77 contains 13,083 utterances with a single banking domain and 77 intents. HWU64 includes 25,716 utterances with 64 intents spanning 21 domains. We follow the setup of \newcite{mehri2020dialoglue}, where a small portion of the training set is separated as a validation set, and the test set is unchanged.  Following previous work, we repeat our few-shot learning model training five times and report the average accuracy. 

\subsection{Model Training and Baselines}

We utilize RoBERTa with {\tt base} configuration, \textit{i.e.}, {\tt roberta-base} as the BERT encoder. We pre-train the combined intent datasets without test sets in the contrastive pre-training stage for 15 epochs, where we set the batch size to 64, $\tau$ to 0.1, and $\lambda$ to 1.0. The pre-training phase takes around 2.5 hours on a single NVIDIA Tesla V100 GPU with 32GB memory. We fine-tune the model under 5-shot (5 training examples per intent) and 10-shot settings (10 training examples per intent). We set the batch size to 16, and do hyper-parameters search for $\tau \,{\in}\, \{0.1, 0.3, 0.5\}$  and $\lambda' \,{\in}\, \{0.01,0.03,0.05\}$; the fine-tuning takes five minutes for each run with 30 epochs. We apply label smoothing to the intent classification loss, following \newcite{zhang2020discriminative}. 

\paragraph{Baselines}
We compare with six strong models. 1, RoBERTa+Classifier~\citep{zhang2020discriminative}: it is a RoBERTa-based classification model. 2, USE~\newcite{yang2020multilingual}: it is the large multilingual model pre-trained on 16 languages. 3, CONVERT~\citep{efficient_intent}: it is an intent detection model with dual encoders, and the dual encoder models are pre-trained on 654 million (input, response) pairs from Reddit. 4, CONVEBERT~\citep{mehri2020dialoglue}: it fine-tunes BERT on a large open-domain dialogue corpus with 700 million conversations. 5, CONVEBERT+Comined~\citep{mehri2020example}: it is an intent detection model based on CONVEBERT, with example-driven training based on similarity matching and observers for transformer attentions. It also conducts task-adaptive self-supervised learning with mask language modeling (MLM) on the intent detection datasets. {\tt Combine} represents the best {\tt MLM+Example+Observers} setting in the referenced paper. 6, DNNC~\citep{zhang2020discriminative}: it is a discriminative nearest-neighbor model which finds the best-matched example from the training set through similarity matching. The model conducts data augmentation during training and boosts performance by pre-training on three natural language inference tasks. 







